The Landscape of Thermal Transients from Supernova Interacting with a Circumstellar Medium

The interaction of supernova ejecta with a surrounding circumstellar medium (CSM) generates a strong shock which can convert the ejecta kinetic energy into observable radiation. Given the diversity of potential CSM structures (arising from diverse mass loss processes such as late-stage stellar outbursts, binary interaction, and winds), the resulting transients can display a wide range of light curve morphologies. We provide a framework for classifying the transients arising from interaction with a spherical CSM shell. The light curves are decomposed into five consecutive phases, starting from the onset of interaction and extending through shock breakout and subsequent shock cooling. The relative prominence of each phase in the light curve is determined by two dimensionless quantities representing the CSM-to-ejecta mass ratio $\eta$, and a breakout parameter $\xi$. These two parameters define four light curve morphology classes, where each class is characterized by the location of shock breakout and the degree of deceleration as the shock sweeps up the CSM. We compile analytic scaling relations connecting the luminosity and duration of each light curve phase to the physical parameters. We then run a grid of radiation hydrodynamics simulations for a wide range of ejecta and CSM parameters to numerically explore the landscape of interaction light curves, and to calibrate and confirm the analytic scalings. We connect our theoretical framework to several case studies of observed transients, highlighting the relevance in explaining slow-rising and superluminous supernovae, fast blue optical transients, and double-peaked light curves.

==> analytics.tex <==


\section{Physical Picture of CSM Shock Breakout}





%DK: Can clarify that this is for a simplified setup; more generally we would also need to describe the ejecta profiles, and any substructure or asymmetry. 
The physical problem of CSM interaction can be generally characterized by 7 dimensionful quantities:
\begin{itemize}
    \item $M_{\rm csm}$ -- total CSM mass
    \item $M_{\rm ej}$ -- total ejecta mass
    \item $R_{\rm csm}$ -- inner CSM radius
    \item $\Delta R_{\rm csm}$ -- CSM width
    \item $v_{\rm ej}$ -- ejecta velocity
    \item $\kappa$ -- opacity
    \item $c$ -- speed of light
\end{itemize}




\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{lc_classes_phases.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}


We can define four dimensionless quantities to describe the problem
\begin{itemize}
    \item $\eta=M_{\rm csm}/M_{\rm ej}$ -- the ratio between the CSM and ejecta mass
    \item $\Delta = \Delta R_{\rm csm}/R_{\rm csm}$ -- the fractional CSM width
    \item $\tau_{\rm csm}=\kappa M_{\rm csm}/R_{\rm csm}^2 \times f(s,\Delta)$ -- the characteristic CSM optical depth.
    \item $\beta=v_{\rm ej}/c$ -- the ejecta velocity relative to $c$
\end{itemize}
where $f(s,\Delta)$ is a geometric correction factor depending on the CSM density profile and width. For constant density ($s=0$) and $\Delta=1$, $f(s,\Delta)=3/28\pi$ (see Appendix).


The light curve depends on various limits of the dimensionless quantities, as they set the behavior of the shock radiation. It is therefore useful to outline the different limiting cases that result for a given choice of dimensionless quantities.


% DK: Would quickly review the basics, that tau R/c is the photon diffusion time and R/v is the shock speed.  When tau < c/v the radiation will leak ahead of the shock and smear it out, a case we refer to as "radiative shock breakout" 

% There is another important event, which is the shock reaching the edge of the CSM.  I think we have called this "shock emergence" or maybe "shock blowout". At this time the energy deposition by the shock will drop sharply. 

% In any case, we can clarify the distinction here.  As I understand, "surface" breakout" corresponds to when the shock breakout is quickly followed by "shock blowout".  We have a venting of the radiation of energy, followed by cooling. Tbe "deep breakouts" correspond to when blowout happens well after blowout, so that when we see the light curve when the forward shock is still going on. 

% Might be good to enumerate these cases when giving the description of these. If I have it right:

% 1) Surface, tau > vej/c 
% 2) Deep obscured, 1 < 1 < vej/c 
% 3) Deep exposed, tau < 1 

% Is the DE case really tau < 1, though? I thought in some cases could have higher tau....




As the ejecta runs into the CSM, the shock decelerates, forming a forward and reverse shock \citep{1982ApJ...258..790C,2019ApJ...884...87T}. The dynamics and escaping radiation of CSM interaction depends sensitively on whether or not a radiation-dominated shock forms. We therefore consider two different regimes: $\tau_{\rm csm}\gg c/v_{\rm sh}$ and $\tau_{\rm csm}<c/v_{\rm sh}$, where $v_{\rm sh}=v_{\rm sh}(t)$ is the instantaneous shock velocity and $v_{\rm sh}(0)=v_{\rm ej}$ (the ejecta decelerates as it sweeps up the CSM).

In the former case ($\tau_{\rm csm}\gg c/v_{\rm sh}$), a radiation-dominated shock is able to form within the CSM, with the shock-deposited thermal radiation unable to diffuse ahead of the shock. The radiation-dominated shock ``dissolves'' once it reaches an optical depth (relative to the outer CSM edge) of $\tau\sim c/v_{\rm sh}$, and radiation is able to escape ahead of the shock. We refer to this scenario as \textbf{surface shock breakout (S)} due to the fact that the shock becomes visible (i.e. radiation escapes) only once it nears the outer edge of the CSM. The physical picture is similar to that seen in shock breakout from a stellar surface (e.g. \cite{1992ApJ...393..742E,1999ApJ...510..379M,2010ApJ...725..904N}).

On the other hand, if $\tau_{\rm csm}<c/v_{\rm sh}$, then a radiation-dominated shock does not form, and the shock-deposited energy diffuses ahead of the shock continuously during interaction. In this case, the shock becomes visible well before reaching the outer CSM edge, and so the shock is effectively buried underneath a layer of unshocked CSM. We refer to this situation as a \textit{deep breakout}, given that the radius of the shock at peak is less than the outer CSM radius. Stated another way, the shock in a deep breakout will have radiated away the majority of its energy by the time it reaches the outer edge of the CSM, while the shock in a surface breakout emits a pulse of radiation at the moment it hits the outer edge.


Note that the CSM can still be optically thick, $\tau_{\rm csm}\gg 1$ to radiation, and so the timescale for the shock to be visible depends on the diffusion time through the unshocked layer. We call the $1< \tau_{\rm csm}<c/v_{\rm sh}$ case a \textbf{deep obscured breakout (DO)}. This scenario can be achieved by several factors. In particular, as $\eta$ increases, the CSM becomes more optically thick ($\tau_{\rm csm}\propto M_{\rm csm}$), increasing the diffusion time. In addition, for $\eta\gg 1$, the ejecta decelerates significantly, and so $v_{\rm sh}$ decreases in time while the breakout optical depth $c/v_{\rm sh}$ increases, thereby pushing the breakout radius deeper into the CSM. Eventually, $v_{\rm sh}$ will drop sufficiently that radiation is able to escape ahead of the shock. Unlike the \textit{surface breakout} scenario whereby the shock becomes visible by reaching the edge of the CSM where $\tau\sim c/v_{\rm sh}$, the shock becomes visible in the \textit{deep obscured breakout} scenario due to the deceleration of the shock. 

For $\tau_{\rm csm}\sim 1$, the shock radiation is able to instantaneously escape through the optically thin CSM, which we refer to as a \textbf{deep exposed breakout (DE)}. In this case, we expect $\eta\ll 1$, and so the ejecta incurs only a minor amount of deceleration ($v_{\rm sh}\approx v_{\rm ej}$). The shock in this case is visible for nearly all of the interaction phase.

In Fig. (?), we show the light curves that result from each of the three breakout scenarios: surface, deep obscured, and deep exposed. The light curve shapes of each class are quite different from each other, as a reuslt of different physics controlling the rise and peak. 

For a surface breakout event, the interaction is effectively ``dark'' until it reaches the outermost breakout layer, where it then rises quickly to peak followed by a fast decline. The deep exposed event is characterized by a fast rise due to an optically thin CSM, with the light curve tracking the instantaneous shock luminosity, i.e. $L(t)\approx L_{\rm sh}(t)$. Finally, the deep obscured event is characterized by a slow rise to peak, with the rise being set by the diffusion timescale through the unshocked optically thick CSM that lies above the shock. 

As a result of these different breakout conditions for the light curve, we must consider each class individually in terms of the physical properties and resulting light curve. In this paper, we focus our analysis on \textit{surface shock breakout} events. We defer a full analysis of the deep breakout events to a follow-up work.


\subsection{Ejecta Properties}
The ejecta can be characterized by the following quantities:
\begin{itemize}
    \item $M_{\rm ej}$ -- total ejecta mass
    \item $E_{\rm sn}$ -- total ejecta energy
    \item $v_{\rm ej}\equiv \sqrt{E_{\rm sn}/M_{\rm ej}}$ -- characteristic ejecta velocity
\end{itemize}
We assume the ejecta is undergoing homologous expansion, and so the velocity profile is given by $v(r,t)=r/t$. 

Next, we must specify the density profile of the ejecta. Following \citep{1989ApJ...341..867C,2016ApJ...821...36K}, we take the ejecta density profile to consist of a broken power law. In particular, the ejecta consists of a shallow inner-density profile with power-law index $\delta$ and a steep outer density profile $n$, with the transition occuring at a velocity coordinate $v_t$:
\begin{align}
\rho_{\rm ej}(r,t) = f_\rho\frac{M_{\rm ej}}{v_t^3 t^3}\left(\frac{r}{v_tt}\right)^{-(n,\delta)}
\end{align}
where
\begin{align}
f_\rho=\frac{(n-3)(3-\delta)}{4\pi(n-\delta)}
\end{align}
The transition velocity coordinate can be expressed in terms of the ejecta mass and energy as
\begin{align}
v_t =f_v\left(\frac{E_{\rm sn}}{M_{\rm ej}}\right)^{1/2}
\end{align}
where
\begin{align}
f_v = \sqrt{\frac{2(5-\delta)(n-5)}{(3-\delta)(n-3)}}
\end{align}
For this work, we take $\delta=0$ and $n=10$ as fiducial values. 

\subsection{CSM Properties}
The CSM can be characterized by the following quantities:
\begin{itemize}
    \item $M_{\rm csm}$ -- total CSM mass
    \item $R_{\rm csm}$ -- inner CSM radius
    \item $\Delta R_{\rm csm}$ -- CSM width
\end{itemize}
The CSM thus extends from $R_{\rm csm}$ to $R_{\rm csm}+\Delta R_{\rm csm}$. The CSM also moves at some characteristic velocity, but here we assume that $v_{\rm csm}\ll v_{\rm ej}$, and so we take $v_{\rm csm}=0$. We note that this may not hold in all cases, where the CSM velocity can be non-negligible (relative to the ejecta velocity) due to e.g. eruptive mass loss episodes.

Next, we construct the CSM density profile. There is a large uncertainty as to the exact structure of the CSM density profile, as it depends sensitively on the mass-loss history of the progenitor. Given this ambiguity, we construct it similarly to the ejecta with a two-component profile: a shallow inner-density CSM shell $\rho_{\rm csm}(r)$ with power-law index $s$, and a steep breakout layer $\rho_{\rm bo}(r)$ with index $p$. The two density profile components are therefore

\begin{align}
    \rho_{\rm csm}(r) = \frac{M_{\rm csm}}{R_{\rm csm}^3}\left(\frac{r}{R_{\rm csm}}\right)^{-s}d(s,\Delta)
&& (R_{\rm csm}\leq r \leq R+\Delta R_{\rm csm})
\end{align} 
where
\begin{align}
    d(s,\Delta)=\frac{3-s}{4\pi}\left[(1+\Delta)^{3-s}-1\right]^{-1}
\end{align}
is a geometric correction factor depending on the CSM density profile.  The breakout layer extends out to a radius $R_{\rm bo}$, and is given by
\begin{align}
    \rho_{\rm bo}(r) = \rho_0^{\rm bo} \left(\frac{r}{R_{\rm csm}+\Delta R_{\rm csm}}\right)^{-p} && (R_{\rm csm}+\Delta R_{\rm csm}<r\leq R_{\rm bo})
\end{align}
where $\rho_0^{\rm bo}=\rho_{\rm csm}(r=R_{\rm csm}+\Delta R_{\rm csm})$. For this work, we choose $p=50$; as we will show, the results are relatively insensitive to the exact value of $p$ as long as it is sufficiently steep (see below).




\section{Analytic Estimates for Surface Shock Breakout}

%DK: Eventually we should add more citations here, since there have been other analytic estimates that followed similar arguments. 
In the following, we assume that shock breakout occurs within the steep outer layer of the CSM. The density profile in the outermost layer goes as
\begin{align}
    \rho(r)=\rho_0\left(\frac{r}{R_*}\right)^{-p}
\end{align}
where $\rho_0\sim M_{\rm csm}/R_{\rm csm}^3$, and $R_*$ is the characteristic radius of the breakout layer. We define \textit{radiative} breakout as when the shock reaches an optical depth $\tau_{\rm bo}=c/v_{\rm bo}$ relative to the outer edge \citep{1999ApJ...510..379M}, where $v_{\rm bo}$ is the shock velocity at breakout. Solving for the (radiative) breakout radius, we get
\begin{align}
    r_{\rm bo}\sim R_*\left[\frac{\rho_0 \kappa R_* v_{\rm bo}}{(p-1)c}\right]^\frac{1}{p-1}
\end{align}
We can similarly find the breakout density $\rho_{\rm bo}=\rho(r_{\rm bo})$ to get
\begin{align}
    \rho_{\rm bo} \sim \rho_0\left[\frac{\rho_0\kappa R_* v_{\rm bo}}{(p-1)c}\right]^{\frac{p}{1-p}}
\end{align}
%DK: I think the above Eq. is wrong? Doesn't look like what you would get if plug r_bo from Eq. 9 into eq 8.
For $p\gg 1$ we get
\begin{align}
    \rho_{\rm bo}\sim \frac{(p-1)c}{\kappa R_* v_{\rm bo}}
\end{align}
% DK: Why not change (p-1) to just p in limit p >> 1

In the case of strong planar shock acceleration  the shock velocity follows the Gandel'Man-Frank-Kamenetskii-Sakurai shock solution \citep{1956SPhD....1..223G,1990ApJ...359..463C,1999ApJ...510..379M,2017hsn..book..967W}
\begin{align}
    v_{\rm sh}\sim v_*\left[\frac{M_{\rm csm}}{\rho r^3}\right]^{\beta}
\end{align}
where $v_*$ is related to the characteristic SN ejecta velocity, and $\beta\approx 0.2$ for a strong shock \citep{2017hsn..book..967W}. Using the density distribution Eq.(?) we get the shock velocity as a function of radius
\begin{align}
    v_{\rm sh}\sim v_*\left[\frac{r}{R_*}\right]^{\beta(p-3)}
\end{align}
%DK: It is a little unclear to me if you are dropping factors here (e.g., factors of 4 pi) and just looking for scalings. If so, maybe state up front. 
Thus, for $p>3$, the shock accelerates while for $p<3$, the shock decelerates. For the breakout density profile Eq. (?) we examine, we are always in the former regime, and so the shock progressively accelerates down the steep outer density profile.

Using $r_{\rm bo}$ from Eq. (?) we can substitute into Eq. (?) to get the shock velocity at the time of breakout
\begin{align}
v_{\rm bo}\sim v_*\left[\frac{(p-1)c}{\rho_0\kappa R_* v_{\rm bo}}\right]^{\beta(p-3)/(1-p)}
\end{align}
Rearranging to solve for the breakout velocity, we get
\begin{align}
v_{\rm bo}\sim v_* \left[\frac{(p-1)c}{\kappa\rho_0 R_*v_*}\right]^\alpha
\end{align}
where
\begin{align}
\alpha = \frac{\beta}{\beta+(1-p)/(p-3)}
\end{align}
For $\beta=0.2$ and $p=50$, we get $\alpha= -0.23$.
%DK: Might mention the limit p-> infinity here, in which case alpha = beta/(beta -1).  So beta = 0.2 gives beta - 0.25.  You might also consider defining alpha as a positive quantity, 

Next, we relate $v_*$ to the SN ejecta velocity $v_{\rm ej}$. Here, we consider the outermost steep layer of the ejecta, where the density goes as
\begin{align}
    \rho_{\rm ej}(r)=\frac{f_\rho M_{\rm ej}}{v_{\rm ej}^3 t^3}\left(\frac{r}{v_{\rm ej}t}\right)^{-n}
\end{align}
The mass contained above a radius $r$ in the ejecta is
\begin{align}
M(r)=4\pi\int_r^\infty r^2\rho_{\rm ej}(r)\,{\rm d}r
\end{align}
Since we assume homologous expansion of the ejecta $v(r)=r/t$ and using Eq.(?), we can similarly define the mass above a velocity $v_0$ in the ejecta as
\begin{align}
M(v_0) = \frac{4\pi}{n-3}f_\rho M_{\rm ej}\left(\frac{v_0}{v_{\rm ej}}\right)^{3-n}
\end{align}
where $n>3$ in order for the mass to be finite.
Similarly, the kinetic energy contained above a radius $r$ in the ejecta is given as
\begin{align}
    E_{\rm kin}(r)=\frac{1}{2}\int_r^\infty 4\pi r^2 \rho_{\rm ej}(r)v(r)^2\,{\rm d}r
\end{align}
Again using the fact that the ejecta is expanding homologously and the density profile Eq.(?), the kinetic energy contained above a velocity $v_0$ in the ejecta is
\begin{align}
E_{\rm kin}(v_0) = \frac{2\pi}{n-5}f_{\rho}M_{\rm ej}v_{\rm ej}^2 \left(\frac{v_0}{v_{\rm ej}}\right)^{5-n}
\end{align}
At the time the shock reaches the breakout layer $R_*$, the ejecta will have interacted with the bulk of the CSM mass. From conservation of momentum, the ejecta kinetic energy that the CSM taps from interaction is roughly
\begin{align}
E_{\rm kin}(v_*)\sim M_{\rm csm}v_*^2
\end{align}
Using Eq.(?) we can solve for the shock velocity at $R_*$ to get
\begin{align}
v_* = K_0 v_{\rm ej}\left(\frac{M_{\rm csm}}{M_{\rm ej}}\right)^{\frac{1}{3-n}}
\end{align}
where $K_0$ is a constant depending on the assumed value of $n$ and $\delta$ of the ejecta.

Going back to Eq.(?), we can substitute in Eq.(?) to get the breakout velocity $v_{\rm bo}$ in terms of the ejecta velocity $v_{\rm ej}$
\begin{align}
v_{\rm bo}\sim v_{\rm ej}^{1-\alpha}\left(\frac{M_{\rm csm}}{M_{\rm ej}}\right)^{\frac{1-\alpha}{3-n}}\left[\frac{(p-1)c}{\kappa\rho_0 R_*}\right]^\alpha
\end{align}

The luminosity at radiative breakout goes as \citep{2017hsn..book..967W}
\begin{align}
L_{\rm bo}\sim 4\pi r_{\rm bo}^2 \rho_{\rm bo}v_{\rm bo}^3
\end{align}
From Eq.(?) we get that $r_{\rm bo}\sim R_*$, assuming that $p$ is sufficiently large that the bracketed term is negligible, and so using Eq.(?)
\begin{align}
L_{\rm bo}\sim \frac{c}{\kappa}R_*v_{\rm bo}^2
\end{align}
Since $\rho_0\sim M_{\rm csm}/R_*^3$ and $R_*\propto R_{\rm csm}$, we get that the breakout luminosity scales as
\begin{align}
L_{\rm bo}\propto R_{\rm csm}^{1+4\alpha}v_{\rm ej}^{2(1-\alpha)}M_{\rm csm}^{\frac{2(1-\alpha)}{3-n}-2\alpha}M_{\rm ej}^{\frac{2(1-\alpha)}{n-3}}\kappa^{-(1+2\alpha)}
\end{align}
The peak luminosity of the light curve will be roughly the luminosity at radiative breakout, and so we get that the peak luminosity goes as
\begin{align}
L_{\rm peak}\propto R_{\rm csm}^{0.05}v_{\rm ej}^{2.5}M_{\rm csm}^{-0.35}M_{\rm ej}^{0.35}\kappa^{-0.53}
\end{align}
 
The radiative efficiency of the shock interaction (i.e. how much of the ejecta kinetic energy is tapped into and radiated away) can be roughly approximated as
\begin{align}
\epsilon_{\rm rad} \sim \frac{L_{\rm p}t_{\rm r}}{M_{\rm ej}v_{\rm ej}^2}
\end{align}
In the case of Type S breakouts, the efficiency goes as
\begin{align}
\epsilon \sim \frac{1}{\beta\tau}
\end{align}
Solving for $t_{\rm r}$ we get
\begin{align}
t_{\rm rise}\sim \frac{M_{\rm ej}R_{\rm csm}^2v_{\rm ej}c}{M_{\rm csm}\kappa L_{\rm p}}
\end{align}
Using Eq.(?) we get
\begin{align}
t_{\rm rise}\propto M_{\rm ej}^{0.65}M_{\rm csm}^{-0.65}R_{\rm csm}^2 v_{\rm ej}^{-1.5}\kappa^{-0.47}
\end{align}

DK: The analysis here is good, though a bit long. We might consider cutting equations to make it more concise, or keeping it step by step but putting the detailed steps in an appendix, 

\subtive efficiency frsectiontion (i.e. h{Com shock interacharacteristic Quantities}
The dynamics of circumstellar interaction will give rise to several characteristic timescales that set the behavior of the underlying light curve. In particular:

\begin{itemize}
    \item \textbf{Expansion Timescale:} $t_{\rm exp}=(R_{\rm csm}-r_0})/v_{\rm ej}$. This is the time relative to explosion it takes for mass extending out to radius $r_0$ expanding with a velocity $v_{\rm ej}$ to begin interacting with the inner edge of the CSM at radius $R_{\rm csm}$. The ejecta can be considered to be in free expansion for this timescale. For a wind extending to e.g. the stellar surface, $t_{\rm exp}=0$. 
    \item \textbf{Dynamical/Shock Crossing Timescale:} $t_0 = \Delta R_{\rm csm}/v_{\rm sh}$. The time it takes for the shock driven by the ejecta to cross the entirety of the CSM. Note that conservation of momentum requires that the shock velocity decreases in time as it sweeps up the CSM, and so $v_{\rm sh}$ is the characteristic shock velocity averaged over the interaction. The shock velocity will scale with the ejecta velocity, $v_{\rm sh}\sim v_{\rm ej}$. In particualr, setting $v_{\rm sh}=v_{\rm ej}$ gives a \textit{lower limit} for the shock crossing timescale. For this work, we set $v_{\rm sh}=v_{\rm ej}$ with some correction factor depending on $\eta$ and the density profiles of the ejecta and CSM. 
    \item \textbf{Radiative Diffusion Timescale:} $t_d=(1+\tau_{\rm csm})\Delta R_{\rm csm}/c$. This is the characteristic time it takes for radiation to diffuse through the CSM and escape, ultimately powering the light curve. For an optically thin CSM, this is simply the light crossing time, $\Delta R_{\rm csm}/c$. Note that this timescale neglects dynamical effects. If the CSM is sufficiently optically thick, then the radiation will instead be transported primarily by shock advection rather than radiative diffusion until the shock reaches an optical depth $\tau_{\rm sh}\sim c/v_{\rm sh}$ relative to the outer edge. In other words, the radiation is carried along with the shock until the diffusion speed exceeds the shock velocity and radiation outpaces the shock.
\end{itemize}

As will be shown, the relative durations of the timescales will set the morphologies of the light curve.

In addition to the timescales, there are characteristic quantities related to the total energy. In particular:
\begin{itemize}
    \item \textbf{Interaction Energy:} $E_0 = \frac{M_{\rm csm}}{M_{\rm ej}+M_{\rm csm}}M_{\rm ej}v_{\rm ej}^2$ The characteristic energy budget of interaction. For $M_{\rm ej}\gg M_{\rm csm}$, this is $E_0\approx M_{\rm csm}v_{\rm ej}^2$; that is, only a fraction of the ejecta energy contained in a layer of mass equal to the CSM mass participates during the interaction. On the other hand, if $M_{\rm csm}\gg M_{\rm ej}$, we have $E_0\approx M_{\rm ej}v_{\rm ej}^2$, and so the bulk of kinetic energy can be tapped into.
    \item \textbf{Kinetic Conversion Efficiency:} $\epsilon=E_{\rm rad}/E_{ej}$, where $E_{\rm ej}\approx M_{\rm ej}v_{\rm ej}^2$. This is the amount of kinetic energy that goes into powering the light curve from both the forward and reverse shock contributions. As noted above, $\epsilon$ will depend on $\eta$. For $\eta>1$, the bulk of the ejecta kinetic energy will be tapped into. Note that this efficiency will be affected by e.g. adiabatic losses, converting the generated energy back into kinetic energy. Another potentially important effect which will be discussed later is the thermalization efficiency of the shock. Before being converted into radiation energy, the kinetic energy is first converted into the internal energy of the gas. This is accomplished via the shock. The gas must then cool via various emission processes, from which the LC sources its power. If gas is not able to efficiently cool, then $\epsilon$ will decrease.
\end{itemize}







Thus, we are left with 4 free parameters that set the behavior of the problem, which we choose to be:
\begin{enumerate}
    \item $\eta=m_0/M_{\rm ej}=M_{\rm csm}/M_{\rm ej}$ -- ratio between the ejecta and CSM mass
    \item $\Delta = \Delta R_{\rm csm}/r_0=\Delta R_{\rm csm}/R_{\rm csm}$ -- fractional CSM width
    \item $\beta^{-1}=v_0/v_{\rm ej}=c/v_{\rm ej}$ -- scaled ejecta velocity
    \item $\tau=\kappa m_0/r_0^2=\kappa M_{\rm csm}/R_{\rm csm}^2$ -- characteristic optical depth
\end{enumerate}
We can rescale the light curve based to characteristic timescales and luminosity. In particular:
\begin{itemize}
    \item  $t_0=\Delta R_{\rm csm}/v_{\rm ej}$: the dynamical or shock crossing time
    \item $t_d=\tau \Delta R_{\rm csm}/c$: the diffusion timescale of the CSM
    \item $L_0=M_{\rm csm} v_{\rm ej}^3/\Delta R_{\rm csm}$: characteristic luminosity
\end{itemize}



    
\begin{enumerate}
    \item $E_{\rm ej}$: The ejecta/explosion energy
    \item $M_{\rm ej}$: The ejecta mass
    \item $M_{\rm csm}$: The CSM mass
    \item $\kappa$: The opacity
    \item $R_{\rm csm}$: The CSM radius
    \item $\Delta R$: The CSM width
\end{enumerate}

We can rescale the above physical variables into a set of self-similar and dimensionless variables
\begin{enumerate}
    \item $\tau_0=\frac{\kappa M_{\rm csm}}{4\pi R_{\rm csm}^2}$: characteristic optical depth
    \item $\eta=\frac{M_{\rm csm}}{M_{\rm ej}}$: ejecta-CSM mass ratio
    \item $v_0=\sqrt{\frac{E_{\rm ej}}{M_{\rm ej}}}$: characteristic velocity
    \item $t_0=\frac{\Delta R}{v_0}$: characteristic/dynamical timescale
    \item $\mathcal{E}_0=M_{\rm csm}v_0^2$: characteristic energy
    \item $\sigma_0=\frac{t_0}{t_d}=\sqrt{\frac{\Delta R^2 c}{\kappa M_{\rm csm}v_0}}$: ratio between the dynamical and diffusion timescales
\end{enumerate}

The rescaled variables are related to the physical variables as follows:
\begin{enumerate}
    \item $\Delta R=v_0t_0$
    \item $\kappa=\frac{\eta v_0^3 t_0^2 c}{\mathcal{E}_0\sigma_0}$
    \item $M_{\rm csm}=\mathcal{E}_0/v_0^2$
    \item $M_{\rm ej}=\mathcal{E}_0/\eta v_0^2$
    \item $E_{\rm ej}=\mathcal{E}_0/\eta$
    \item $R_{\rm csm}=\sqrt{\frac{\eta v_0 t_0^2 c}{4\pi\sigma_0\tau_0}}$
\end{enumerate}
%
\vspace{1in}
Another way of writing it -- We can choose the code units of our simulation to be
\begin{enumerate}
    \item $r_0 = R_{\rm csm}$
    \item $v_0 = v_{\rm ej}$
    \item $m_0 = M_{\rm ej}$~~(or~~$ m_0 = M_{\rm csm}$)
\end{enumerate}
Then the other code units are derivable
\begin{enumerate}
    \item $t_0 = r_0/v_0$
    \item $\rho_0 = m_0/r_0^3$
    \item $E_0 = m_0 v_0^2$
\end{enumerate}
And we need to run simulations for different values of the dimensionless parameters
\begin{enumerate}
    \item $\eta=\frac{M_{\rm csm}}{M_{\rm ej}}$: ejecta-CSM mass ratio
    \item $\sigma =\frac{t_0}{t_d}=\sqrt{\frac{\Delta R^2 c}{\kappa M_{\rm csm}v_0}}$: ratio between the dynamical and diffusion timescales
    \item $\delta = \Delta R/R_{\rm csm}$: fraactional thickness of csm
\end{enumerate}
Does that capture it? The idea is that for specified values of $\eta, \sigma, \delta$ we just need to setup and run one calculation in code units (e.g., the CSM in our input model starts at $r=1$ and the maximum ejecta velocity is $v = 1$). Then we can derive the values for everything else by just changing the scales (e.g., we multiply the simulation output velocities by $v_{\rm ej}$ to get physical units).

\subsection{Scalings}

The description of the problem has 7 dimensionful parameters
\begin{enumerate}
\item $M_{\rm csm}$
\item $M_{\rm ej}$
\item $R_{\rm csm}$
\item $\Delta R$
\item $v_{\rm ej}$
\item $\kappa$
\item $c$ (speed of light)
\end{enumerate}
(I believe we need to add the speed of light because it appears in the equations once radiation transport is added).

We can choose 3 variables to define our code units, for example
\begin{enumerate}
\item $m_0 = M_{\rm csm}$
\item $r_0 = R_{\rm csm}$
\item $v_0 = v_{\rm ej}$
\end{enumerate}
All other units are (I believe) derivable from these 3. In particular 
\begin{enumerate}
\item $t_0 = r_0/v_0 = R_{\rm csm}/v_{\rm ej}$
\item $\kappa_0 = r_0^2/m_0 = R_{\rm csm}^2/M_{\rm csm}$~
\end{enumerate}

That means we are left with 4 of our 7 parameters, which can be written out dimensionlessly
\begin{enumerate}
\item $\eta= {M_{\rm ej}/m_0 = {M_{\rm ej}/M_{\rm csm}$
\item $\Delta =  \Delta R/r_0 = \Delta R/R_{\rm csm}$
\item $\beta^{-1} =  c/v_0 = c/v_{\rm ej}$
\item $\tau = \kappa/\kappa_0 
= \kappa M_{\rm csm}/R_{\rm csm}^2
$
\end{enumerate}
The last parameter is seen to be
a measure of  optical depth (the exact optical 
depth will vary by some numerical factor depending on the density structure of the gas). We could if we want define a $\sigma$ parameter by combining $\beta$ and $\tau$ -- this may be a nicer approach, not sure.

It is presumably the case that when things are very optically thin, the value of $\tau$ does not matter -- radiation just free streams away from the gas and the value of $\kappa$ is irrelevant. Alternatively, when things are very optically thick everywhere, the value of $\beta$ presumably does not matter. Light cannot free-stream so it's speed is set by diffusion, not by $c$. But for in between cases, we need to do a calculation for different values of $\tau$ and $\beta$.






==> classes.tex <==
\section{Light Curve Classification}
\begin{deluxetable}{ccccc}
\tablehead
{\colhead{} & \colhead{Narrow Lines?} & \colhead{Rise Time} & \colhead{Decline Time} & \colhead{Transient Type}}
\startdata
\textbf{Type DO} & \checkmark & Slow & Slow & SLSN \\
\textbf{Type DE} & \checkmark & Varies & Varies & Ibn/IIn \\
\textbf{Type S} & \ding{55} & Fast & Fast & FBOTs
\enddata
\end{deluxetable}





In theory, all five light curve phases outlined above will be present for any ejecta-CSM configuration. However, the duration of each phase and, therefore, the overall evolution of the LC, will depend on the specifics of ejecta and CSM parameters. In certain cases, one or several of the LC phases outlined in the previous section may be absent or very short. This is especially important when analyzing e.g. peak behavior, as the phase that sets the peak will be different depending on the CSM-ejecta properties, and so the physical scalings of $L_{\rm peak}$ and $t_{\rm peak}$ with e.g. $M_{\rm csm}$ or $M_{\rm ej}$ will differ.

We classify the CSM interaction light curves based on the time when the shock within the CSM ``emerges'', or first becomes visible to an observer (in the form of escaping radiation). Constructed this way, there are 3 possible light curves:
\begin{enumerate}
    \item \textbf{Deep Obscured Emergence (Type DO):} The shock propagates through an optically thick CSM, but becomes visible \textit{before} it reaches the outer edge of the CSM (i.e. shock breakout). In this case, the \textit{radiative breakout phase} dominates the LC.
    \item \textbf{Deep Exposed Emergence (Type DE):} The shock propagates through an optically \textit{thin} CSM, and so the instantaneous shock heating is immediately radiated away. Thus, the \textit{continued interaction phase} dominates.
    \item \textbf{Surface Shock Emergence (Type S):} Radiation is unable to escape from the CSM for the bulk of the interaction, and so the shock becomes visible only once it reaches the outermost edge of the CSM in the \textit{shock breakout phase}. This class is physically similar to the picture of stellar surface shock breakout.
\end{enumerate}
Given that different phases dominate the LC for each class, we consider each individually in terms of understanding the overall LC behavior (e.g. in deriving peak scalings with CSM/ejecta properties). However, it is worth pointing out that certain CSM interaction LCs might not cleanly fall into a specific class, which we call transitional types. 



\begin{deluxetable*}{cccccc}
\tablehead
{\colhead{} & \colhead{Dark Phase} & \colhead{Radiative Breakout} & \colhead{Continued Interaction} & \colhead{Shock Breakout} & \colhead{Cooling + Reverse Shock}}
\startdata
\textbf{Type DO} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\textbf{Type DE} & * &  & \checkmark & \checkmark & * \\
\textbf{Type S} & \checkmark & \checkmark &  & \checkmark & \checkmark
\enddata
\end{deluxetable*}
% \begin{itemize}
%     \item \textbf{Deep Shock Emergence (D):} The radiation escapes ahead of the shock \textit{before} it has completely swept up the CSM.
% \begin{itemize}
%     \item \textbf{Deep Exposed (DE):} The shock propagates through an optically thin CSM, and so the radiative breakout phase is short, and the LC is dominated by the continued interaction phase.
%     \item \textbf{Deep Obscured (DO):} The shock propagates through an optically thick CSM, but is visible before it reaches the outer edge of the CSM. In this case, the radiative breakout phase will dominate the LC, with a continued interaction phase following afterwards.
% \end{itemize}
%     \item \textbf{Surace Shock Emergence (S):} Radiation is visible only once the shock reaches the outermost layers of the CSM (akin to stellar shock breakout).
% \end{itemize}



% \subsection{Type DO: Deep Obscured Shock Emergence}
% A deep obscured shock emergence event (``Type DO'') will generally display all phases of the interaction event, from the dark phase to a reverse shock tail. Such an event arises in the case of a highly optically thick and extended CSM, such that the shock radiation must diffuse out through an optically thick unshocked layer. The LC will feature a dark phase until sufficient time has elapsed that the initial shock heating diffuses out, which is then followed by a smooth rise to peak. For LCs of this type, the peak is set by radiative breakout \textit{within} the CSM, and so is effectively ``obscured'' by the unshocked layer. 

% Once the radiative breakout heating has sufficiently escaped, the LC will then track a continued interaction phase from the previously unshocked CSM that obscured the breakout radiation. This will appear as a flattening in the LC post peak. Given that the LC is dominated by the instantaneous interaction heating rate, the LC will be sensitive to the density structure of the CSM and may contain ``bumps'', unlike the relatively smooth radiative breakout phase. 

% ...

% ...


% Type DE events will display narrow lines in their spectra until shock breakout, and such features may appear relatively strong given the large mass of unshocked CSM necessary to produce such events. The photospheric radius will likely differ from the position of the shock, instead being in some layer within the unshocked CSM. Thus, the photospheric radius will be relatively constant until shock breakout, and will then track the swept-up CSM shell until sufficient time has elapsed for the shell to become optically thin either from expansion or recombination. 

% \subsection{Type DE: Deep Exposed Shock Emergence}

% \subsection{Type S: Surface Shock Emergence}
% A surface shock emergence event occurs when the shock rapidly crosses an optically thick CSM such that radiation is only able to escape once the shock reaches the outer edge of the CSM. The resulting light curve is characterized by an extended dark phase throughout the entirety of interaction, followed by a rapid rise to peak and a sharp drop from shock breakout. In addition, the LC has a late-time tail resulting from reverse shock emission. A surface shock emergence event is characterized by  (1) $\beta\tau\gg 1$ and (2) $\eta<1$. 

% Due to the fast interaction, a continued interaction phase is absent from the light curve. Instead, there exists only a radiative breakout rise followed immediately by a shock breakout drop. The light curve peak is set by the coincidence of radiative and shock breakout. The rapid expansion and cooling of shock breakout leads to a sharp drop onto a reverse shock-powered tail that persists much longer than the breakout phase. 

% The physical conditions most likely to give rise to a Type S interaction event are a dense compact CSM shell (to give a large $\tau$) with a relatively fast ejecta (i.e. a large $\beta$) to satisfy the $\beta\tau>1$ condition. Thus, such events are indicative of an unsteady mass-loss event immediately prior to explosion, rather than an extended dense wind.

% Given the large optical depth of the CSM shell, it is possible that any underlying heating from the ejecta (e.g. stellar shock breakout or radioactive heating) will be obscured and trapped in the CSM, and so such events may ``hide'' the underlying transient, especially if the interaction generates much greater luminosity. If the reverse shock tail weakens or inefficiently thermalizes, then it is possible that any underlying radioactive nickel decay will dominate the light curve. The LC itself is unlikely to provide enough information to distiniguish between reverse shock emission or radioactive heating at late times; in such cases, spectra will be useful in discriminating the source of the heating (e.g. absorption features characteristic of ejecta composition). 

% The photospheric evolution of Type S interaction events will be characterized by an increasing photospheric radius, as the photosphere will track the swept up CSM shell at the outer edge of the ejecta, as well as a decreasing photospheric temperature as the shocked CSM cools. Due to the lack of a continued interaction phase and high shock temperature, the spectra will likely show little to no narrow lines (unless there exists an overlying wind above the shell). It is possible if caught early enough along the radiative breakout rise, the light curve may show narrow lines from the thin unshocked layer before breakout. In general, though, the spectra will appear relatively featureless with a blue continuum.

% Since the LC is dominated by the breakout phase (radiative+shock), the LC shape is relatively insensitive to the shape of the CSM shell (e.g. a constant vs. decreasing density profile), as the LC becomes visible only once the majority of the CSM has been swept up. The shock breakout fall might be impacted by how steep the outer CSM edge is, with a more gradual tapering giving a slower decline. 

% \textcolor{blue}{Fiducial Model: $M_{\rm ej}=3M_\odot$, $M_{\rm csm}=0.3M_\odot$, $v_{\rm ej}=10^4$ km s$^{-1}$, $\kappa=0.4$ cm$^2$ g$^{-1}$, $R_{\rm csm}=5\cdot 10^{13}$ cm, $\Delta R_{\rm csm}=10^{13}$ cm, $s=0$, $h=0.01$, $\epsilon=10^{-3}$.}

==> introduction.tex <==
\section{Introduction}





The usual picture of supernova light curves comes from a combination of neutrino-driven shock cooling and/or the radioactive decay of $^{56}$Ni; the photons diffuse out of an expanding ejecta; the diversity of ejecta properties and explosion energies produces a wide range of light curve durations and luminosities. Recent all-sky observations have enlarged the domain of transient types, uncovering highly luminous events outside of the realm of ``typical'' supernovae. These events occur on timescales as short as a few hours, to as long as several months. Their extreme brightness and gamut of timescales challenge usual explanations of energetic transients.

In core-collapse supernovae, half of the explosion energy is converted into thermal energy from the passage of a strong neutrino-driven shock. Due to the high optical depths of stellar interiors, most of this energy is lost to adiabatic expansion of the ejecta. The other half of the explosion energy is stored in a reservoir of kinetic energy of order $\sim 10^{51}$ ergs. If this prodigious store of energy can be tapped into and converted into observable electromagnetic radiation, then they will be able of powering some of the most energetic events in the transient sky.

Shocks provide the physical mechanism with which we can extract kinetic energy and power a light curve through the means of the second law of thermodynamics: viscous shock passage converts kinetic energy into internal energy of the gas. If the shock is optically thin, then a \textit{collisionless shock} forms and most of the kinetic energy remains as internal gas energy. This is typically the case for supernova remnants. While such sites are expected to be efficient sources of energetic cosmic rays and non-thermal radio/X-ray emission, they are incapable of powering luminous optical transients that are being discovered. Instead, these events require the formation of a \textit{radiative} shock. 

The formation of such shocks requires the pesence of a circumstellar medium (CSM) that is moving slowly relative to the ejecta velocity. Supernova ejecta masses are typically only a fraction of the zero age main-sequence mass of the star, losing their outer layers through several potential mass-loss mechanisms. Much of the mass will be shed throughout the star's life in the form of a stellar wind, escaping the stellar environment and entering the interstellar medium. In order to power the aforementioned shocks, the mass loss must instead be located within the immediate vicinity of the stellar progenitor, which means the mass loss must occur shortly before supernova. Furthermore, the mass loss has to be a significant fraction of the ejecta mass in order to effectively tap the ejecta kinetic energy, as well as produce the conditions necessary for radiative shock formation. These mass loss events are often referred in the literature as stellar outbursts, and numerous explanations have been proposed regarding their origin, ranging from binary interaction to unstable nuclear burning.



Observations of stellar outbursts and supernova spectra motivate the plausibility of ``circumstellar interaction'' as a viable explanation for at least some of the transient duration-luminosity space. Given the ubiquity of mass loss and supernova rates, they are an appealing mechanism for unusual supernovae, including superluminous events and the recently emerging class of so-called fast blue optical transients (FBOTs). 

The properties of circumstellar interaction have been extensively researched in the literature, and has gained popularity in recent times to explain superluminous events and the so-called fast blue optical transients (FBOTs). These include several numerical and analytical works to predict the light curve and spectra of CSM interaction, as well as fits to specific events. 

In this work, we give an illustrative picture of circumstellar interaction and construct a theoretical framework with which to analyze their light curves, with the aid of numerical radiation hydrodynamics simulations. In particular, we show how circumstellar interaction produces a wide diversity of light curve morphologies set by the shockwave physics, and how each light curve can be decomposed into a series of consecutive phases that are uniquely determined by the ejecta and CSM properties. We show how each phase can be used to glean information regarding the interaction, and reduce the expected light curve type to a set of three dimensionless parameters.

In Section 2 we give a qualitative overview of CSM interaction, and the basic physics of the light curve. We then give a more quantitative analysis in Sec 3, including useful scaling relations for each phase, which we compare with numerical simulations. Finally, in Sec. 4, we show how the results can be used to infer properties of the CSM mass and radius, and the applicability of different interaction scenarios to observed transient phenomena. For clarity of text, we provide a more complete description of the numerics and supplementary euations in the Appendix.
